GPU Domain Specialization via Composable On-Package Architecture

As GPUs scale their low precision matrix math throughput to boost deep learning (DL) performance, they upset the balance between math throughput and memory system capabilities. We demonstrate that converged GPU design trying to address diverging architectural requirements between FP32 (or larger) based HPC and FP16 (or smaller) based DL workloads results in sub-optimal configuration for either of the application domains. We argue that a Composable On-PAckage GPU (COPAGPU) architecture to provide domain-specialized GPU products is the most practical solution to these diverging requirements. A COPA-GPU leverages multi-chip-module disaggregation to support maximal design reuse, along with memory system specialization per application domain. We show how a COPA-GPU enables DL-specialized products by modular augmentation of the baseline GPU architecture with up to 4x higher off-die bandwidth, 32x larger on-package cache, 2.3x higher DRAM bandwidth and capacity, while conveniently supporting scaled-down HPC-oriented designs. This work explores the microarchitectural design necessary to enable composable GPUs and evaluates the benefits composability can provide to HPC, DL training, and DL inference. We show that when compared to a converged GPU design, a DL-optimized COPA-GPU featuring a combination of 16x larger cache capacity and 1.6x higher DRAM bandwidth scales per-GPU training and inference performance by 31% and 35% respectively and reduces the number of GPU instances by 50% in scale-out training scenarios.

==> eval-hpc.tex <==
% \subsection{HPC-optimized COPA-GPU Evaluation}
\begin{figure}[t]
    \center
    \includegraphics[width=1\linewidth, trim= 0 0 0 0,clip]{./figures/gpun_hpc_drambw.pdf}
    \vspace{-0.2in}
    \caption{Normalized performance of HPC-optimized COPA-GPU on 130 HPC applications versus off-chip DRAM bandwidth.}
    \label{fig:dram_bw_hpc}
    \vspace{-0.2in}
\end{figure}

Since we have demonstrated that memory bandwidth for the baseline GPU-N is under-utilized for most HPC applications,
HPC-optimized COPA-GPU architecture focuses on weakening the memory system rather than augmenting it for the purpose 
of cost saving. Figure~\ref{fig:dram_bw_hpc} shows the normalized performance of HPC-optimized COPA-GPU across all 130
HPC applications under different DRAM bandwidth settings. As shown in the figure, most HPC applications are
insensitive to either DRAM bandwidth increase or decrease. When DRAM bandwidth is increased to infinite, a geomean speedup of only 5\% is achieved.
 When DRAM bandwidth is decreased, 0.83$\times$BW, 0.75$\times$BW and 0.67$\times$BW result in 3\%, 4\% and 7\% geomean slowdown, respectively.
Therefore, we believe HPC-optimized COPA-GPUs can be designed with reduced DRAM bandwidth with minimal performance degradation.

%%TODO: For Nil to explain different options to reduce DRAM bandwidth.
A GPU with reduced peak DRAM bandwidth can be derived from the
baseline GPU in several ways. The first option is to reduce the
operating frequency of the baseline HBM
system in proportion with the desired reduction in bandwidth, but
retain the same number of HBM stacks and hence channels. The obvious
benefits of this design are that DRAM capacity and the GPU die layout
and architecture are unchanged, aiding composability. However this
approach does not reduce cost, and despite the reduction in frequency, does not
appreciably reduce the DRAM power consumption. This is
because DRAM core voltage is already at the lowest possible level
(with guardbands), so no further voltage reduction with quadratic
power savings are feasible. The reduced frequency of the DRAM I/Os,
while beneficial, has marginal impact on overall power since the
fraction of I/O power in HBM is much lower than in GDDR5. And further,
standby power is mostly due to refresh which is unaffected by the
frequency. Alternatively, two different cost-optimized architectures
are possible. The first is to reduce the bandwidth by reducing the
number of stacks, reducing DRAM cost but also reducing memory
capacity. For example, 0.83$\times$BW and 0.67$\times$BW would correspond to 
reducing the number of stacks from 6 to 5 and 4, respectively, in our proposed COPA-GPU architectures.
Considering that the model sizes of DL applications are growing much faster
than the working set sizes of HPC applications, we believe it is most cost-effecitive
for the HPC-optimized COPA-GPU to have lower memory capacity than what a DL-optimized COPA-GPU has.
The other solution is to retain the same number of channels and frame buffer
design, but utilize HBM devices from a previous generation that have a
lower peak operating frequency, but also lower cost due to volume
production. An example of this is the HBM2 technology used in NVIDIA 40GB-A100~\cite{ampere} results in 25\%
DRAM bandwidth reduction compared to the HBM2e technology used in the latest NVIDIA 80GB-A100~\cite{ampere_80gb}. 
 


==> eval.tex <==
\vspace{-0.05in}
\input{bottleneck.tex}

\begin{table}[t]
    \centering
    \small
    \renewcommand\tabcolsep{3pt}
        \begin{tabular}{|l|c|c|c|}
         \hline
        Architecture   & LLC capacity & DRAM BW & DRAM capacity \\ 
        configuration  & (MB) & (TB/s) & (GB) \\\hline
        GPU-N         & 60                & 2.7              & 216    \\ \hline
        HBM+L3        & 960               & 2.7              & 216    \\ \hline
        HBML+L3       & 960               & 4.5              & 360    \\ \hline
        HBM+L3L       & 1920              & 2.7              & 216    \\ \hline
        HBML+L3L      & 1920              & 4.5              & 360    \\ \hline
        HBMLL+L3L     & 1920              & 6.3              & 504    \\ \hline
        Perfect L2   & infinite          & infinite         & infinite  \\ \hline
        \end{tabular}
    \caption{COPA-GPU architectural parameters.}
    \label{tab:arch}
    \vspace{-0.2in}
\end{table}


% UHB link requirements and contrasts them
% to the technology projections in
% Section~\ref{sec:sec:copa-gpu-technologies}\@. Then we evaluate six
% domain-specialized COPA-GPU configurations and compare their
% performance using the MLPerf training and inference benchmarks.
% Finally, we analyze the DL-specialized COPA-GPU strong-scaling
% efficiency when compared to scaling-out DL training with larger
% multi-GPU installations of baseline GPU-Ns\@.

{\bf COPA-GPU Configurations}
Table~\ref{tab:arch} summarizes a set of DL-optimized COPA-GPU
configurations that are enabled by architectural choices outlined in
Section~\ref{sec:arch}. The DL-optimized HBM+L3 COPA-GPU design
provides 960MB of L3 cache through either 3D stacking with a single
maximum-sized MSM die, or 2.5D stacking with two MSM dies, each set to
half of the maximum die size. The option with more HBM resources, denoted by
an HBML in the HBML+L3, applies only to 2.5D, by exploiting the extra
MSM die edge area to provide 1.7$\times$ higher HBM bandwidth and a
larger HBM capacity (10 HBM sites in total). If we equip 2 maximum-sized
MSM dies under 2.5D stacking scenario, the L3 cache capacity can be further doubled to 1920MB
along with more MSM die edge area which enables increasing the number of HBM sites to
2.3$\times$ that of the baseline (14 HBM sites in total). Therefore, we add three more
configurations with 1920MB of L3 cache and various HBM resources: HBM+L3L, HBML+L3L and HBMLL+L3L.



\begin{figure}[t]
  \center
  \includegraphics[width=1\linewidth]{./figures/gpun_l3bw.pdf}
\caption{Geomean HBM+L3 COPA-GPU performance versus UHB link bandwidth to the
L3 cache.}
\label{fig:l3_bw}
\vspace{-0.2in}
\end{figure}

{\bf UHB Link Bandwidth and Latency}
We first examine the on-package UHB link bandwidth requirements by sweeping
the unidirectional L3 bandwidth in the HBM+L3 configuration from half of its original
DRAM bandwidth (0.5$\times$RD+0.5$\times$WR which sums to 2.7TB/s) up
to infinite bandwidth. Figure~\ref{fig:l3_bw} summarizes the
geometric mean performance speedups of the MLPerf applications (training and
inference), normalized to the baseline GPU-N (without L3)\@. The
performance increases dramatically when the L3 bandwidth grows from
0.5$\times$RD+0.5$\times$WR to 2$\times$RD+2$\times$WR, with
diminishing returns beyond that point. Overall, the UHB bandwidth
configurations of 2$\times$RD+2$\times$WR (total 10.8TB/s) comes
within 3\% and 6\% of the infinite bandwidth settings for training
and inference respectively. Our previous analysis indicates that this
bandwidth is well within the capabilities of the 2.5/3D technologies
(Section~\ref{sec:sec:copa-gpu-technologies}). 

We also examine the effect of UHB link latency by varying the total
round-trip latency between L2 and L3 from 0.25$\times$ to 1$\times$ of
the DRAM access latency. Our experiments (not shown) indicate that
COPA-GPU is not sensitive to L3 latency, as performance changes
by less than 2\% across this latency range.  For the rest of this
paper, we set the UHB link bandwidth to be 2$\times$RD+2$\times$WR,
for a total of 10.8TB/s and the round-trip latency between L2 and L3
(UHB link latency plus L3 access latency) to be half the DRAM access
latency.


\begin{figure*}[t]
  \begin{subfigure}[t]{1\textwidth}
    \center
    \includegraphics[width=1\linewidth]{./figures/gpun_train_arch.pdf}
    \caption{Training}
    \label{fig:perf_arch_train}
  \end{subfigure}
  \begin{subfigure}[t]{1\textwidth}
    \center
    \includegraphics[width=1\linewidth]{./figures/gpun_inference_arch.pdf}
    \caption{Inference}
    \label{fig:perf_arch_inference}
  \end{subfigure}
\caption{The MLPerf training and inference performance on DL-optimized COPA-GPUs
with varying designs, normalized to the
baseline GPU-N performance. Large-batch and small-batch cases are
denoted by \textit{lb} and \textit{sb}.}
\label{fig:perf_arch}
\vspace{-0.2in}
\end{figure*}

{\bf Performance Evaluation}
Figure~\ref{fig:perf_arch} summarizes
the MLPerf training and inference performance of the COPA-GPU designs
from Table~\ref{tab:arch}, in both large batch (\textit{lb}), and
small batch (\textit{sb}) settings.
The larger cache and memory capabilities each improve both large-batch
and small-batch training performance. For example, the additional
cache in the HBM+L3 configuration improves large-batch and small-batch
performance by 21\% and 18\% respectively, making it a very attractive
3D COPA-GPU design. The additional HBM bandwidth in the HBML+L3
configuration achieves an overall 31\% and 27\% speedup, making it a
very attractive 2.5D COPA-GPU design choice. HBM+L3L performs worse than 
HBML+L3 by 4\% at both large-batch and small batch, indicating increasing
L3 capacity alone is not the best solution to speedup training performance.
More ambitious options such as HBML+L3L and HBMLL+L3L only lead to within 4\% marginal 
gains compared to HBML+L3, which does not justify the additional cost. We also
add a perfect L2 setting where all L2 requests always hit as an upper bound comparison.


As large-batch inference is primarily limited by DRAM
bandwidth, a large L3 is very effective at lowering off-chip
traffic. Larger cache capacity in HBM+L3 improves performance by 29\%,
and HBM+L3L can reach speedup as high as 40\%. With 1920MB of L3, further increasing HBM
bandwidth is not beneficial anymore as most of the DRAM traffic has already been filtered 
out by the large L3 cache. In fact, although not shown in the figure, we found that the DRAM
bandwidth can be even reduced by 50\% without affecting the performance. Large-batch inference benefits more from caching
than DL training, however because small-batch inference performance is
capped by low GPU SM utilization rather than DRAM bandwidth (due to the fact that 60MB L2 baseline
is sufficient to capture most data on-chip for small-batch inference), the
performance improvement via the combination of L3 and HBM is just
9\%. Overall, our results show that HBML+L3 is likely the best COPA design that works well for
both DL training and inference workloads as it achieves similar performance to more costly options at lower
cost. Inference is more sensitive to LLC capacity and less sensitive to DRAM bandwidth than training in general, so trading
HBM resources with more LLC capacity is desirable if we would like to further optimize a COPA-GPU design solely for DL inference.

In terms of power efficiency, COPA-GPU L3 reduces the total DRAM-related per-GPU energy consumption by up to 3.4$\times$ with HBM and 5.6$\times$ with off-package DDR as shown in Section~\ref{sec:sec:uarch}. 
Overall the improved DL-optimized COPA-GPU performance may lead to increased power that may or may not be fully mitigated by the significant power reduction in the memory system. To mitigate that growing thermal density, we expect future high-end GPU systems to rely on liquid cooling technologies to enable substantially higher thermal envelopes than possible today~\cite{GoogleCooling,LiquidCooledSpec}.


{\bf Scale-out Training Efficiency}
Multi-GPU training performance is eventually limited by decreasing 
per-GPU compute efficiency and growing
system-level synchronization overheads. To study the scale-out
efficiency of DL-optimized COPA-GPUs, we compared the performance
of a COPA-GPU based system with 2$\times$ and 4$\times$ larger
systems consisting of the baseline GPU-Ns. We keep the global batch
size constant across all configurations to maintain the same
statistical efficiency~\cite{hp_micro_2019}. Consequently, the per-GPU
batch size drops to one half and one quarter for the baseline GPU-N
configurations. We also did not extrapolate the additional overheads of
a larger distributed gradient synchronization. Thus, our analysis is conservative,
favoring the 2$\times$ and 4$\times$ GPU-N configurations.

Shown in Figure~\ref{fig:2dp}, doubling and quadrupling the number of
baseline GPU-N instances (2$\times$ GPU-Ns and 4$\times$ GPU-Ns)
results in mean 29\% and 43\% performance gains, respectively for our
training workloads. The DL-optimized HBML+L3 COPA-GPU configuration provides
similar levels of performance to 2$\times$ GPU-Ns, yet
cost significantly less than buying 2$\times$ more the traditional GPUs.

When compared to GPU-N, HBML+L3 doubles the silicon area by adding close to 826mm$^2$ of silicon with largely regular SRAM-based cache arrays and interconnect that are expected to achieve higher manufacturing yields due to built in redundancy and error recovery mechanisms, compared to the GPU die with complex logic. Moreover, this area is split into two smaller dies, resulting in substantially lower cost per mm$^2$. 
In terms of costly HBM resources, HBML+L3 integrates only 1.6$\times$ more HBM memory, resulting in total cost significantly lower than 2$\times$ of GPU-N. We conclude that DL-optimized COPA-GPUs will provide substantially better cost-performance at scale, saving not just
overall GPU cost but additional system-level collateral, such as
datacenter floorspace, CPUs, network switches, and other
peripheral devices.


% In {\it maskrcnn}, the COPA-GPU approach is more efficient as the per-GPU batch size is
% already one, and further data parallelism cannot be applied.
% For applications such as {\it minigo} and {\it ncf} that
% only scale to tens of GPUs, the 2$\times$ GPU-Ns and
% 4$\times$ GPU-Ns cases achieve significant performance gains since we
% do not account for the inter-node gradient synchronization
% overheads. Finally, for memory-intensive applications such as {\it
% gnmt} and {\it transformer}, further data parallelism provides only
% limited performance gains. DL-optimized COPA-GPU configurations
% can achieve much better performance gain even compared to the
% 4$\times$ GPU-Ns\@.



%old
% Figure~\ref{fig:2dp} shows that doubling and quadrupling the number of
% baseline GPU-N instances (2$\times$ GPU-Ns and 4$\times$ GPU-Ns)
% result in mean 29\% and 43\% performance gains, respectively. As a
% comparison, the DL-optimized COPA-GPU configurations provide similar
% levels of speedups while featuring 2$\times$ and 4$\times$ fewer node
% counts. For instance, HBML+L3 comes within 2\% of the 2$\times$
% GPU-Ns case. HBML+L3L outperforms 2$\times$ GPU-Ns case by 4\% and comes
% within 10\% of the 4$\times$ GPU-Ns case. In {\it maskrcnn}, because
% the per-GPU batch size is already one, further data parallelism cannot
% be applied and the COPA-GPU approach is more
% efficient. For applications such as {\it minigo} and {\it ncf} that
% only scale to tens of GPUs, the 2$\times$ GPU-Ns and
% 4$\times$ GPU-Ns cases achieve significant performance gains since we
% do not account for the inter-node gradient synchronization
% overheads. Finally, for memory-intensive applications such as {\it
% gnmt} and {\it transformer}, further data parallelism provides only
% limited performance gains. DL-optimized COPA-GPU configurations
% can achieve much better performance gain even compared to the
% 4$\times$ larger cluster of GPU-Ns\@. We conclude that COPA-GPUs can be
% performance-competitive with larger multi-GPU installations, saving
% GPU counts as well as additional system-level costs, such as
% datacenter floorspace, CPUs, network switches, connectors, and other
% peripheral devices.




==> scaling_dram_capacity.tex <==
{\bf Scaling GPU DRAM Capacity.} Future GPUs will need to improve
capacity in tandem with performance for emerging large DL
models~\cite{msft_zero, guptajeanwu_facebook_recommender}. However,
the evolutionary scaling of HBM devices is unlikely to provide the
necessary capacity. According to the HBM2 JEDEC specification, DRAM
die density and stacking technology improvements can yield 8-high stacks
of 32Gb dies. Six stacks of such 36GB HBM devices can be used to equip
GPU-N with a maximum of 216GB of memory, while ten and fourteen stacks in the DL-optimized variant
of the 2.5D COPA-GPU can have 360GB and 504GB of capacity. 

%\Comment{SK: This next paragraph is not well integrated into the story. We have a diagram in Figure 6
%showing 10 stacks of HBM and it isn't clear how the bandwidth targets
%below fit into the earlier story. Also - does this tie into the rest
%of the paper later - or is it just a side note about alternative DRAM
%technologies?}

However the COPA-GPU architecture enables a path to even higher DRAM
capacity for future GPUs. The large on-package SRAM bandwidth enabled
by the COPA-GPU architecture can reduce the off-package bandwidth
demand, allowing the use of 
lower-bandwidth, but denser off-package commodity DRAMs\@. For
example, the HBM stacks could be replaced by a larger on-GPU LLC
backed by a memory system consisting solely of future LPDDR devices.
As a case study, a current high-end graphics GPU (RTX-2080-Ti) is
provisioned with 600GB/s of off-package GDDR6 memory~\cite{turing}\@.
Assuming current x64 LPDDR5 DRAMs with 51.2GB/s of bandwidth and 16GB
capacity per device, a GPU with 600GB/s could be provisioned with 12
LPDDR devices and 192GB of total capacity.  However, the lower per pin
bandwidth of LPDDR5 (8Gb/s~\cite{halee20_lp5} versus 14Gb/s for
GDDR6~\cite{turing}) requires 1.7$\times$ more pins than GDDR6 to
provide the same bandwidth.  

The 2$\times$ larger package of 2.5D
COPA-GPU can readily accommodate this demand, while the 3D COPA-GPU
design will likely require a bigger package to enjoy the benefits of
higher memory capacity. Assuming the same 1.7$\times$ scaling of LPDDR
bandwidth as assumed for HBM (see Table~\ref{tab:gpu_trend}), a
2.5D COPA-GPU system with 1 TB/s of aggregate bandwidth could be
constructed from 12 future LPDDR devices. With DRAM density doubling
to 32Gb per die, this system can have 384GB of capacity. However, if the same
bandwidth is provisioned using twenty-four x32 devices that have half the
bandwidth of their x64 counterparts, the capacity can be increased to
768GB. We evaluate the performance characteristics of such
LPDDR-based COPA-GPUs in Section~\ref{sec:performance_evaluation}.

%\Comment{SK: I don't understand the math - what's the bandwidth of a
%octa-die package - are you still assuming 51.2GB/s? Need to make this
%calculation more obvious.} By choosing from x64 or x32 parts, a 1TB/s
%LPDDR-based COPA-GPU can therefore provide either 368GB or 736GB of
%total DRAM capacity.


%To support the needs of large DL
%models~\cite{msft_zero,guptajeanwu_facebook_recommender}, DL-oriented GPUs would
%ideally improve both memory capacity and bandwidth. However, significant
%improvements in memory capacity through the evolutionary scaling of HBM is
%unlikely. Current 16GB HBM2 devices are 8-high stacks of 16Gb DRAM dies. The
%HBM2E JEDEC specification~\cite{jedec_hbm} projects 12-high stacks at a maximum,
%with 16Gb DRAM dies expected to scale to 24 or 32Gb\@. Thus, current 16GB HBM2
%stacks can be scaled to a maximum capacity of 36 or 48 GB in the future.

%The COPA-GPU organization enables higher per-GPU DRAM capacity by deployment of
%higher capacity DRAM devices belonging to the lower power DDR (LPDDR) family of
%DRAMs. These DRAMs have not typically been used with GPUs because their lower
%bandwidth cannot meet the needs of HPC or graphics applications.
%Section~\ref{sec:eval} evaluates COPA-GPU configurations where the HBM memory is
%replaced by LPDDR-based devices. This work assumes that the
%minimum total off-package bandwidth in LPDDR-based GPUs will be similar to a
%%modern GDDR6-based device, such as the RTX-2080-Ti, i.e., 600
%GB/s~\cite{turing}\@.  However, the lower per pin bandwidth of LPDDR5
%(8Gb/s~\cite{halee20_lp5}) compared to GDDR6 (14Gb/s~\cite{turing}) requires
%1.75$\times$ more pins to support the same bandwidth.  The 2$\times$ larger
%package of 2D COPA-GPU can readily accommodate this demand, while the 3D
%COPA-GPU design will likely require a bigger package to enjoy the benefits of
%higher memory capacity.

%Current LPDDR5 devices are $\times$64, octa-die packages with 16GB capacity and
%51.2GB/s of bandwidth. A 600GB/s COPA-GPU provisioned with such LPDDR5 devices
%will have 187GB of total DRAM capacity. Future LPDDR5 interfaces will operate at
%8Gb/s~\cite{halee20_lp5}, and the LPDDR5 dies, will scale to 32Gb densities.
%Therefore, a future $\times$64 LPDDR5 octa-die device will have 64GB/s of
%bandwidth and 32GB of capacity. As is commonly the case, we can also expect a
%$\times$32 version of this device with the same capacity and half the bandwidth
%(32GB/s)\@. A 600GB/s COPA-GPU architecture can choose between these different
%bandwidth-to-capacity ratios to trade-off cost and capability, and be can
%provisioned with either 300GB ($\times$64 device) or 600GB ($\times$32 device)
%of capacity.
%\Comment{YF:Need to project one generation further with memory BW scaling
%rate of 1.7x so that 600GB would become 1TB.}


